A precision measurement of the e+p/e-p elastic scattering cross section ratio at the OLYMPUS experiment

Measurements of the ratio of the proton elastic form factors ($\mu_pG_E/G_M$) using Rosenbluth separation and those using polarization-based techniques show a strong discrepancy, which has persisted both in modern experimental results and in re-analyses of previous data. The most widely accepted hypothesis to explain this discrepancy is the treatment of the contributions from hard two-photon exchange (TPE) to elastic electron-proton scattering in the radiative corrections applied to the Rosenbluth separation measurements. Calculations of the hard TPE contribution are highly model dependent, but the effect may be measured experimentally with a precise determination of the ratio of the positron-proton and electron-proton elastic scattering cross sections. The OLYMPUS experiment collected approximately 4 fb$^{-1}$ of \pp and \ep scattering data at the DORIS storage ring at DESY in 2012, with the goal of measuring the elastic \ratio ratio over the kinematic range $(0.4 \leq \epsilon \leq 0.9)$, $(0.6 \leq Q^2 \leq 2.2)$ GeV$^2/c^2$ at a fixed lepton beam energy of 2.01 GeV. The detector for the OLYMPUS experiment consisted of refurbished elements of the Bates Large Acceptance Spectrometer Toroid (BLAST) surrounding an internal gaseous hydrogen target, with the addition of multiple systems for the monitoring of the luminosity collected by the experiment. A detailed simulation of the experiment was developed to account for both radiative corrections and various systematic effects. This work presents preliminary results from the OLYMPUS data, demonstrating that the elastic \ratio ratio rises to several percent at $\epsilon\approx 0.4$ and indicating a significant contribution from TPE to \pmp scattering. Additionally, the value of \ratio has been measured to unprecedented precision at $\epsilon=0.98$, which provides a valuable normalization point for other experimental data.

==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Physics as follows:

\signature{Professor Jianshu Cao}{Chairman, Thesis Committee \\
   Professor of Physics}

\signature{Professor Troy Van Voorhis}{Thesis Supervisor \\
   Associate Professor of Physics}

\signature{Professor Robert W. Field}{Member, Thesis Committee \\
   Haslam and Dewey Professor of Physics}
\end{large}
\end{titlepage}


